Towards String-to-Tree Neural Machine Translation

We present a simple method to incorporate syntactic information about the target language in a neural machine translation system by translating into linearized, lexicalized constituency trees. An experiment on the WMT16 German-English news translation task resulted in an improved BLEU score when compared to a syntax-agnostic NMT baseline trained on the same dataset. An analysis of the translations from the syntax-aware system shows that it performs more reordering during translation in comparison to the baseline. A small-scale human evaluation also showed an advantage to the syntax-aware system.

==> old_table.tex <==
\begin{tabular}{ll|l}
\hline
src      & \multicolumn{2}{l}{ ...habe ich gemerkt, dass ich zwar meinen Kopf steuern, aber meinen Korper nicht tauschen kann, \underline{erklärte} Glandorf...} \\
ref      & \multicolumn{2}{l}{...I realized that I was able to control my head, but I couldn't play tricks with my body," he explained in...} \\
2tree & \multicolumn{2}{l}{...I noticed that while \textcolor{blue}{I control my head, I can't deceive my body}", Glandorf explained in the interview...} \\
2bpe  & \multicolumn{2}{l}{...I noticed that while \textcolor{red}{I'm steering my head, but my body can't fool}", Glandorf explained in the interview... }\\ \hline

src      & Wie Pastor Martin Luther King Jr. vor fünfzig Jahren \underline{sagte:} & Jetzt \underline{ist} keine Spur der Tumore mehr sichtbar.\\
ref      & As the Reverend Martin Luther King Jr. said fifty years ago: \\
2tree & As Pastor Martin Luther King Jr. \textcolor{blue}{said fifty years ago}: \\
2bpe  & As Pastor Martin Luther King Jr. \textcolor{red}{fifty years ago said}: \\ \hline
src      & Jetzt \underline{ist} keine Spur der Tumore mehr sichtbar.\\
ref      & Now there is no sign of the tumours. \\
2tree & Now \textcolor{blue}{there is} no trace of tumors.\\
2bpe  & Now no trace of \textcolor{blue}{the} tumors \textcolor{red}{is more} visible. \\ \hline

src      & Mit die größte Schwierigkeit \underline{war} der Perspektivwechsel von der Position eines Arztes zu der eines Patienten.\\
ref      & One of the hardest things was moving from the position of doctor to that of patient. \\
2tree & The greatest difficulty \textbf{was} the change of perspective from the position of a doctor \textcolor{blue}{to that} of a patient.\\
2bpe  & With the greatest difficulty, the change of perspective \textbf{was} from a doctor's position \textcolor{red}{on that} of a patient. \\ \hline

src      & Ailinn \underline{verstand} das nicht.\\
ref      & Ailinn didn't understand. \\
2tree & Ailinn \textcolor{blue}{did not understand this}.\\
2bpe  & Ailinn \textcolor{red}{understood this not}. \\ \hline

% src      & Darunter ist ein Azubi, der bereits zuvor eine andere Ausbildung in dem Unternehmen abgeschlossen hat.\\
% ref      & They include a trainee, who had already completed another course in the same company. \\
% 2tree & Among them is a \textcolor{blue}{trainee} who has already completed another course of education in the company.\\
% 2bpe  & Among them is a \textcolor{red}{Azubi}, who has already completed a different training in the company. \\ \hline

% src      & Wir müssen für einen friedlichen Himmel kämpfen.\\
% ref      & We must fight for a peaceful sky. \\
% 2tree & We must fight for a peaceful \textcolor{blue}{sky}.\\
% 2bpe  & We must fight for a peaceful \textcolor{red}{heaven}. \\ \hline

% TODO add back at camera-ready
%src      & Es \underline{muss} für ihn noch viel heftiger sein, weil er dort war und ich nicht.\\
%ref      & It must be even stronger for him because he was there and I was not. \\
%2tree & It has to be much stronger for him because he was there and \textcolor{blue}{I was not}.\\
%2bpe  & It must be much more intense for him because he was there and \textcolor{red}{I don't}. \\ \hline

src      & Auf Webseiten \underline{wird} das Thema Asbest in Schulen jetzt häufig angesprochen.\\
ref      & Websites have sprung up to address the issue of asbestos in schools. \\
2tree & On web pages, the issue of \textcolor{blue}{asbestos in schools} is frequently mentioned now.\\
2bpe  & On websites, the issue of asbestos is now frequently \textcolor{red}{addressed in schools.} \\ \hline


src      & \parbox[t]{13cm}{Huthi \underline{drohte} nach Angaben des Blattes mit einer weiteren Eskalation des Konflikts, sollten seine\\ Forderungen nicht erfüllt werden.}\\
ref      & The report said that Huthi threatened further escalation of the conflict, should his demands not be met. \\
2tree & According to the leaf, Huthi threatened with a further escalation of the conflict \textcolor{blue}{if its demands were not met.} \\
2bpe  & Huthi, threatened \textcolor{red}{by} the hand of a further escalation of the conflict, \textcolor{red}{should not meet his demands}. \\ \hline

src      & Ich \underline{kann} kaum glauben, dass ich einige Stunden lang so sicher war, dass er tot sei und ich ihn nie wieder sehen würde.\\
ref      & I can hardly believe that for some hours I was so sure he was dead and I'd never see him again. \\
2tree & I can't believe that for a few hours I have been so sure he is dead and that \textcolor{blue}{I would} never see it again. \\
2bpe  & I can hardly believe that I have been so sure for a few hours that he is dead \textcolor{red}{and never see} him again.
 \\ \hline

\end{tabular}
